Tree-Independent Dual-Tree Algorithms

Dual-tree algorithms are a widely used class of branch-and-bound algorithms. Unfortunately, developing dual-tree algorithms for use with different trees and problems is often complex and burdensome. We introduce a four-part logical split: the tree, the traversal, the point-to-point base case, and the pruning rule. We provide a meta-algorithm which allows development of dual-tree algorithms in a tree-independent manner and easy extension to entirely new types of trees. Representations are provided for five common algorithms; for k-nearest neighbor search, this leads to a novel, tighter pruning bound. The meta-algorithm also allows straightforward extensions to massively parallel settings.

==> boruvka-a.tex <==
\begin{tikzpicture}[scale=0.9]
  % Axes.
%  \coordinate (Origin) at (0, 0);
%  \coordinate (XAxisMin) at (0, 0);
%  \coordinate (XAxisMax) at (2.5, 0);
%  \coordinate (YAxisMin) at (0, 0);
%  \coordinate (YAxisMax) at (0, 3.5);
%  \draw [thin, gray, -latex] (XAxisMin) -- (XAxisMax);
%  \draw [thin, gray, -latex] (YAxisMin) -- (YAxisMax);

  % Points x_1 to x_10.
  \node [draw, circle, inner sep=1pt, fill] at (0, 0.25) { };
%  \node [ ] at (0.45, 0.05) { $x_1$ };

  \node [draw, circle, inner sep=1pt, fill] at (0.5, 0.25) { };
%  \node [ ] at (0.95, 0.05) { $x_2$ };

  \node [draw, circle, inner sep=1pt, fill] at (0, 1.25) { };
%  \node [ ] at (0.45, 1.05) { $x_3$ };

  \node [draw, circle, inner sep=1pt, fill] at (0, 3.25) { };
%  \node [ ] at (0.25, 2.95) { $x_4$ };

  \node [draw, circle, inner sep=1pt, fill] at (1, 3.25) { };
%  \node [ ] at (1.45, 3.05) { $x_5$ };

  \node [draw, circle, inner sep=1pt, fill] at (0.75, 2.75) { };
%  \node [ ] at (1.2, 2.55) { $x_6$ };

  \node [draw, circle, inner sep=1pt, fill] at (2, 0.25) { };
%  \node [ ] at (2.45, 0.05) { $x_7$ };

  \node [draw, circle, inner sep=1pt, fill] at (2, 0.75) { };
%  \node [ ] at (2.25, 0.95) { $x_8$ };

  \node [draw, circle, inner sep=1pt, fill] at (2, 3.25) { };
%  \node [ ] at (2.55, 3.05) { $x_9$ };

  \node [draw, circle, inner sep=1pt, fill] at (2, 2.5) { };
%  \node [ ] at (2.45, 2.3) { $x_{10}$ };

  % component c_1
  \draw [thin] (0, 0.25) -- (0.5, 0.25);
  \draw [thin] (0, 0.25) -- (0, 1.25);

  \node [ ] at (0.35, 0.5) { $c_1$ };

  % component c_2
  \draw [thin] (0, 3.25) -- (0.75, 2.75);
  \draw [thin] (0.75, 2.75) -- (1, 3.25);

  \node [ ] at (0.5, 3.25) { $c_2$ };

  % component c_3
  \draw [thin] (2, 0.25) -- (2.0, 0.75);

  \node [ ] at (1.75, 0.5) { $c_3$ };

  % component c_4
  \draw [thin] (2.0, 3.25) -- (2.0, 2.5);

  \node [ ] at (1.75, 2.8) { $c_4$ };

  \draw [thin, gray] (2.5, 0.25) -- (2.5, 3.25);

\end{tikzpicture}


==> boruvka-b.tex <==
\begin{tikzpicture}[scale=0.9]
  % Axes.
%  \coordinate (Origin) at (0, 0);
%  \coordinate (XAxisMin) at (0, 0);
%  \coordinate (XAxisMax) at (2.5, 0);
%  \coordinate (YAxisMin) at (0, 0);
%  \coordinate (YAxisMax) at (0, 3.5);
%  \draw [thin, -latex] (XAxisMin) -- (XAxisMax);
%  \draw [thin, -latex] (YAxisMin) -- (YAxisMax);

  % Points x_1 to x_10.
  \node [draw, circle, inner sep=1pt, fill] at (0, 0.25) { };
%  \node [ ] at (0.45, 0.05) { $x_1$ };

  \node [draw, circle, inner sep=1pt, fill] at (0.5, 0.25) { };
%  \node [ ] at (0.95, 0.05) { $x_2$ };

  \node [draw, circle, inner sep=1pt, fill] at (0, 1.25) { };
%  \node [ ] at (0.45, 1.05) { $x_3$ };

  \node [draw, circle, inner sep=1pt, fill] at (0, 3.25) { };
%  \node [ ] at (0.25, 2.95) { $x_4$ };

  \node [draw, circle, inner sep=1pt, fill] at (1, 3.25) { };
%  \node [ ] at (1.45, 3.05) { $x_5$ };

  \node [draw, circle, inner sep=1pt, fill] at (0.75, 2.75) { };
%  \node [ ] at (1.2, 2.55) { $x_6$ };

  \node [draw, circle, inner sep=1pt, fill] at (2, 0.25) { };
%  \node [ ] at (2.45, 0.05) { $x_7$ };

  \node [draw, circle, inner sep=1pt, fill] at (2, 0.75) { };
%  \node [ ] at (2.25, 0.95) { $x_8$ };

  \node [draw, circle, inner sep=1pt, fill] at (2, 3.25) { };
%  \node [ ] at (2.55, 3.05) { $x_9$ };

  \node [draw, circle, inner sep=1pt, fill] at (2, 2.5) { };
%  \node [ ] at (2.45, 2.3) { $x_{10}$ };

  % component c_5
  \draw [thin] (0, 0.25) -- (0.5, 0.25);
  \draw [thin] (0, 0.25) -- (0, 1.25);
  \draw [thin] (2, 0.25) -- (2, 0.75);

  \draw [thin] (0.5, 0.25) -- (2, 0.25);
  \node [ ] at (1, 0.5) { $c_5$ };

  % component c_6
  \draw [thin] (0, 3.25) -- (0.75, 2.75);
  \draw [thin] (0.75, 2.75) -- (1, 3.25);
  \draw [thin] (2, 3.25) -- (2, 2.5);

  \draw [thin] (1, 3.25) -- (2, 3.25);
  \node [ ] at (1.5, 2.8) { $c_6$ };

  \draw [thin, gray] (2.5, 0.25) -- (2.5, 3.25);

\end{tikzpicture}


==> boruvka-c.tex <==
\begin{tikzpicture}[scale=0.9]
  % Axes.
%  \coordinate (Origin) at (0, 0);
%  \coordinate (XAxisMin) at (0, 0);
%  \coordinate (XAxisMax) at (2.5, 0);
%  \coordinate (YAxisMin) at (0, 0);
%  \coordinate (YAxisMax) at (0, 3.5);
%  \draw [thin, -latex] (XAxisMin) -- (XAxisMax);
%  \draw [thin, -latex] (YAxisMin) -- (YAxisMax);

  % Points x_1 to x_10.
  \node [draw, circle, inner sep=1pt, fill] at (0, 0.25) { };
%  \node [ ] at (0.45, 0.05) { $x_1$ };

  \node [draw, circle, inner sep=1pt, fill] at (0.5, 0.25) { };
%  \node [ ] at (0.95, 0.05) { $x_2$ };

  \node [draw, circle, inner sep=1pt, fill] at (0, 1.25) { };
%  \node [ ] at (0.45, 1.05) { $x_3$ };

  \node [draw, circle, inner sep=1pt, fill] at (0, 3.25) { };
%  \node [ ] at (0.25, 2.95) { $x_4$ };

  \node [draw, circle, inner sep=1pt, fill] at (1, 3.25) { };
%  \node [ ] at (1.45, 3.05) { $x_5$ };

  \node [draw, circle, inner sep=1pt, fill] at (0.75, 2.75) { };
%  \node [ ] at (1.2, 2.55) { $x_6$ };

  \node [draw, circle, inner sep=1pt, fill] at (2, 0.25) { };
%  \node [ ] at (2.45, 0.05) { $x_7$ };

  \node [draw, circle, inner sep=1pt, fill] at (2, 0.75) { };
%  \node [ ] at (2.25, 0.95) { $x_8$ };

  \node [draw, circle, inner sep=1pt, fill] at (2, 3.25) { };
%  \node [ ] at (2.55, 3.05) { $x_9$ };

  \node [draw, circle, inner sep=1pt, fill] at (2, 2.5) { };
%  \node [ ] at (2.45, 2.3) { $x_{10}$ };

  \draw [thin] (0, 0.25) -- (0.5, 0.25);
  \draw [thin] (0, 0.25) -- (0, 1.25);
  \draw [thin] (2, 0.25) -- (2, 0.75);

  \draw [thin] (0, 3.25) -- (0.75, 2.75);
  \draw [thin] (0.75, 2.75) -- (1, 3.25);
  \draw [thin] (2, 3.25) -- (2, 2.5);

  \draw [thin] (0.5, 0.25) -- (2, 0.25);
  \draw [thin] (1, 3.25) -- (2, 3.25);

  \draw [thin] (0, 1.25) -- (0.75, 2.75);


\end{tikzpicture}

